Setting Optimal Reserve Prices using Fine-Tuned Language Models

Online auction houses must set reserve prices for highly differentiated products whose unstructured descriptions contain valuable demand information. Existing approaches generally require managers to specify product attributes in advance. We ask whether a language model can instead learn from listing descriptions and historical bids to set item-specific reserve prices before bidding begins. We fine-tune a pretrained text embedding language model using the structural likelihood of auction bids as its training objective. This directs representation learning toward the valuation distribution that determines the reserve decision. We show that consecutive upper bids identify the tail information needed to set an optimal reserve without observing or modeling the number of potential bidders. A split-sample estimator learns the representation on one half of the data and conducts structural estimation and inference conditional on that representation on the other. We apply the method to approximately 65,800 online used-vehicle auctions. With seller values calibrated to match the sale rate among listings, the model implies a counterfactual net increase of $165.8 million, representing a 14.6% increase above the incumbent reserve policy. The framework translates a listing description and a seller's value into an item-specific reserve recommendation without constructing a product taxonomy or requiring a bid history for the item being priced. It provides an approach to adapting language models for operational decisions in marketplaces where products are heterogeneous and demand-relevant information is recorded in text.

==> figures/data/mileage_elasticity_labels.tex <==
% Generated by mileage_gradient.py -- do not edit by hand.
\pgfplotsset{mileage elasticity ticks/.style={ytick={4,3,2,1}, yticklabels={Second-highest bid,Reserve,Tail intercept,Tail markup}}}


==> figures/data/reserve_policy_bars.tex <==
% Generated by reserve_policy_figure.py -- do not edit by hand.
\addplot[xbar, fill=black!35, draw=none, forget plot] coordinates {(1134.033,5) [1,134.0]};
\addplot[xbar, fill=blue!60!black, draw=none, forget plot] coordinates {(266.723,4) [266.7]};
\addplot[xbar, fill=red!70!black, draw=none, forget plot] coordinates {(100.969,3) [101.0]};
\addplot[xbar, fill=black, draw=none, forget plot] coordinates {(165.754,2) [165.8 (14.6\% of incumbent)]};
\addplot[xbar, fill=blue!60!black!35, draw=none, forget plot] coordinates {(167.267,1) [167.3]};


==> figures/data/reserve_policy_labels.tex <==
% Generated by reserve_policy_figure.py -- do not edit by hand.
\def\RPolSoldAgree{14,007}
\def\RPolSoldBelow{4,194}
\def\RPolSoldBelowReserve{4,194}
\def\RPolSoldBelowNoReserve{0}
\def\RPolUnsoldMet{4,194}
\def\RPolUnsoldAgree{2,778}
\def\RPolN{32,853}
\def\RPolCStar{0.467}
\def\RPolGained{266.7}
\def\RPolLost{101.0}
\def\RPolNet{165.8}
\def\RPolIncumbent{1,134.0}
\def\RPolNetShare{14.6}
\def\RPolUpper{167.3}
\pgfplotsset{reserve policy bar ticks/.style={ytick={5,4,3,2,1}, yticklabels={Incumbent revenue,Final bids gained,Revenue lost,Net revenue,{Payoff gain (upper bound)}}}}


==> figures/data/tails_featured_overlay.tex <==
% Generated by results_exhibits.py -- do not edit by hand.
% Featured listing 64929 fitted inverse hazard over its threshold support band.
% The line v - v0 uses the calibrated seller value.
% The filled marker shows the reserve with its 95% sampling interval.
\addplot[black, line width=1pt, forget plot] coordinates {(12.528,4.8352) (64.000,7.3150)};
\addplot[black, line width=0.6pt, forget plot] coordinates {(13.043,0) (73.043,60)};
\addplot[black, line width=1.2pt, forget plot] coordinates {(17.860,5.1060) (18.439,5.1060)};
\addplot[only marks, mark=*, mark size=1.8pt, black, forget plot] coordinates {(18.149,5.1060)};
\node[anchor=south east, font=\scriptsize] at (axis cs:35.04,21.50) {$v-v_0$};


==> figures/data/tails_panel_a_lines.tex <==
% Generated by results_exhibits.py -- do not edit by hand.
% 400 inference-half listings, rng seed 20260901; colour = divRedWhiteBlue at
% t = 0.5 + 0.5 (xi - 0.1430) / 0.0902, clipped to [0,1], darkened 30%.
\addplot[color={rgb,1:red,0.652;green,0.652;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.500,2.4790) (27.362,6.0368)};
\addplot[color={rgb,1:red,0.463;green,0.463;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.955,4.4549) (68.170,15.0753)};
\addplot[color={rgb,1:red,0.540;green,0.540;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.200,3.5427) (66.393,13.5532)};
\addplot[color={rgb,1:red,0.340;green,0.340;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.855,4.1556) (35.225,9.7183)};
\addplot[color={rgb,1:red,0.316;green,0.316;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.767,3.2614) (66.816,15.1990)};
\addplot[color={rgb,1:red,0.700;green,0.519;blue,0.519}, line width=0.3pt, forget plot] coordinates {(5.878,3.1883) (40.112,7.2845)};
\addplot[color={rgb,1:red,0.484;green,0.484;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.755,3.7630) (96.175,19.0381)};
\addplot[color={rgb,1:red,0.048;green,0.048;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.766,4.0632) (102.000,25.9090)};
\addplot[color={rgb,1:red,0.603;green,0.603;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.755,6.0647) (57.675,13.6671)};
\addplot[color={rgb,1:red,0.497;green,0.497;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.100,3.3554) (46.542,10.1975)};
\addplot[color={rgb,1:red,0.446;green,0.446;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.200,3.8126) (59.725,13.3935)};
\addplot[color={rgb,1:red,0.306;green,0.306;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.655,3.4318) (50.862,12.1873)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.100,3.5345) (80.500,21.9110)};
\addplot[color={rgb,1:red,0.089;green,0.089;blue,0.700}, line width=0.3pt, forget plot] coordinates {(11.000,8.2275) (122.575,32.9637)};
\addplot[color={rgb,1:red,0.028;green,0.028;blue,0.700}, line width=0.3pt, forget plot] coordinates {(12.250,7.2208) (166.450,42.6167)};
\addplot[color={rgb,1:red,0.661;green,0.661;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.741,4.1886) (50.725,10.6964)};
\addplot[color={rgb,1:red,0.526;green,0.526;blue,0.700}, line width=0.3pt, forget plot] coordinates {(14.000,9.2597) (135.270,29.3104)};
\addplot[color={rgb,1:red,0.080;green,0.080;blue,0.700}, line width=0.3pt, forget plot] coordinates {(10.000,7.4071) (113.450,30.4687)};
\addplot[color={rgb,1:red,0.700;green,0.522;blue,0.522}, line width=0.3pt, forget plot] coordinates {(6.300,4.0227) (63.450,10.8817)};
\addplot[color={rgb,1:red,0.513;green,0.513;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.300,3.8416) (89.450,17.7315)};
\addplot[color={rgb,1:red,0.148;green,0.148;blue,0.700}, line width=0.3pt, forget plot] coordinates {(1.555,1.7235) (45.450,11.1190)};
\addplot[color={rgb,1:red,0.229;green,0.229;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.100,3.9820) (75.000,18.0101)};
\addplot[color={rgb,1:red,0.621;green,0.621;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.155,3.0154) (45.575,9.3584)};
\addplot[color={rgb,1:red,0.185;green,0.185;blue,0.700}, line width=0.3pt, forget plot] coordinates {(12.112,6.9102) (157.046,37.2438)};
\addplot[color={rgb,1:red,0.700;green,0.673;blue,0.673}, line width=0.3pt, forget plot] coordinates {(5.500,3.4875) (49.725,9.6558)};
\addplot[color={rgb,1:red,0.675;green,0.675;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.055,4.1022) (63.225,12.4585)};
\addplot[color={rgb,1:red,0.700;green,0.670;blue,0.670}, line width=0.3pt, forget plot] coordinates {(7.921,3.9123) (77.225,13.5495)};
\addplot[color={rgb,1:red,0.430;green,0.430;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.000,5.0663) (92.000,20.0003)};
\addplot[color={rgb,1:red,0.171;green,0.171;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.578,3.4910) (77.125,18.5995)};
\addplot[color={rgb,1:red,0.492;green,0.492;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.310,4.3386) (45.000,10.9058)};
\addplot[color={rgb,1:red,0.320;green,0.320;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.600,2.7416) (37.041,8.9695)};
\addplot[color={rgb,1:red,0.700;green,0.524;blue,0.524}, line width=0.3pt, forget plot] coordinates {(3.898,2.8161) (27.562,5.6609)};
\addplot[color={rgb,1:red,0.700;green,0.687;blue,0.687}, line width=0.3pt, forget plot] coordinates {(3.850,2.4527) (51.410,9.1695)};
\addplot[color={rgb,1:red,0.500;green,0.500;blue,0.700}, line width=0.3pt, forget plot] coordinates {(9.183,5.6175) (105.900,21.9378)};
\addplot[color={rgb,1:red,0.562;green,0.562;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.000,4.2502) (67.041,14.0644)};
\addplot[color={rgb,1:red,0.632;green,0.632;blue,0.700}, line width=0.3pt, forget plot] coordinates {(10.250,5.9223) (92.000,18.3263)};
\addplot[color={rgb,1:red,0.700;green,0.459;blue,0.459}, line width=0.3pt, forget plot] coordinates {(7.883,4.8136) (75.000,12.3256)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(15.275,11.2163) (174.500,52.2762)};
\addplot[color={rgb,1:red,0.676;green,0.676;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.555,2.8380) (49.900,9.3127)};
\addplot[color={rgb,1:red,0.700;green,0.532;blue,0.532}, line width=0.3pt, forget plot] coordinates {(6.328,4.0515) (70.000,11.7775)};
\addplot[color={rgb,1:red,0.697;green,0.697;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.665,4.8085) (101.800,18.1642)};
\addplot[color={rgb,1:red,0.370;green,0.370;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.214,2.8530) (53.175,11.9377)};
\addplot[color={rgb,1:red,0.700;green,0.528;blue,0.528}, line width=0.3pt, forget plot] coordinates {(8.755,5.7109) (83.225,14.7091)};
\addplot[color={rgb,1:red,0.261;green,0.261;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.600,4.1149) (62.000,15.5695)};
\addplot[color={rgb,1:red,0.466;green,0.466;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.555,2.4324) (59.450,11.9368)};
\addplot[color={rgb,1:red,0.638;green,0.638;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.378,1.7706) (21.615,4.6732)};
\addplot[color={rgb,1:red,0.031;green,0.031;blue,0.700}, line width=0.3pt, forget plot] coordinates {(18.000,8.7241) (129.800,34.3439)};
\addplot[color={rgb,1:red,0.700;green,0.487;blue,0.487}, line width=0.3pt, forget plot] coordinates {(3.750,2.9673) (31.225,6.1421)};
\addplot[color={rgb,1:red,0.462;green,0.462;blue,0.700}, line width=0.3pt, forget plot] coordinates {(10.500,6.3948) (85.500,19.4138)};
\addplot[color={rgb,1:red,0.517;green,0.517;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.000,4.7700) (109.700,21.7057)};
\addplot[color={rgb,1:red,0.700;green,0.414;blue,0.414}, line width=0.3pt, forget plot] coordinates {(7.678,5.0191) (68.725,11.4950)};
\addplot[color={rgb,1:red,0.700;green,0.529;blue,0.529}, line width=0.3pt, forget plot] coordinates {(3.850,2.4589) (30.272,5.6533)};
\addplot[color={rgb,1:red,0.700;green,0.585;blue,0.585}, line width=0.3pt, forget plot] coordinates {(9.700,5.6413) (81.225,14.8101)};
\addplot[color={rgb,1:red,0.337;green,0.337;blue,0.700}, line width=0.3pt, forget plot] coordinates {(12.638,7.0244) (117.266,26.8814)};
\addplot[color={rgb,1:red,0.647;green,0.647;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.936,3.7478) (57.788,11.6635)};
\addplot[color={rgb,1:red,0.613;green,0.613;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.800,3.0363) (38.250,8.3489)};
\addplot[color={rgb,1:red,0.700;green,0.683;blue,0.683}, line width=0.3pt, forget plot] coordinates {(13.638,6.0692) (85.000,16.1159)};
\addplot[color={rgb,1:red,0.308;green,0.308;blue,0.700}, line width=0.3pt, forget plot] coordinates {(12.888,10.1089) (105.450,28.0219)};
\addplot[color={rgb,1:red,0.700;green,0.479;blue,0.479}, line width=0.3pt, forget plot] coordinates {(4.620,2.6235) (38.975,6.5560)};
\addplot[color={rgb,1:red,0.589;green,0.589;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.500,4.8626) (50.000,11.5482)};
\addplot[color={rgb,1:red,0.700;green,0.666;blue,0.666}, line width=0.3pt, forget plot] coordinates {(7.000,4.3006) (73.625,13.5356)};
\addplot[color={rgb,1:red,0.700;green,0.652;blue,0.652}, line width=0.3pt, forget plot] coordinates {(3.578,2.4861) (39.112,7.3444)};
\addplot[color={rgb,1:red,0.136;green,0.136;blue,0.700}, line width=0.3pt, forget plot] coordinates {(10.433,8.5704) (144.175,37.4071)};
\addplot[color={rgb,1:red,0.415;green,0.415;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.678,2.8161) (38.862,8.9598)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.700,2.9486) (51.450,16.9737)};
\addplot[color={rgb,1:red,0.556;green,0.556;blue,0.700}, line width=0.3pt, forget plot] coordinates {(9.210,6.7821) (88.445,19.5818)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.155,3.5997) (90.450,27.7722)};
\addplot[color={rgb,1:red,0.343;green,0.343;blue,0.700}, line width=0.3pt, forget plot] coordinates {(11.388,8.4639) (129.900,30.8653)};
\addplot[color={rgb,1:red,0.499;green,0.499;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.800,6.0499) (95.000,20.7743)};
\addplot[color={rgb,1:red,0.470;green,0.470;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.104,5.2943) (77.500,17.6144)};
\addplot[color={rgb,1:red,0.552;green,0.552;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.478,4.3719) (69.725,14.6165)};
\addplot[color={rgb,1:red,0.450;green,0.450;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.416,2.6980) (46.000,9.8056)};
\addplot[color={rgb,1:red,0.700;green,0.620;blue,0.620}, line width=0.3pt, forget plot] coordinates {(19.750,8.0835) (98.075,18.4763)};
\addplot[color={rgb,1:red,0.495;green,0.495;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.000,4.6833) (90.900,19.0579)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.750,2.3765) (43.450,13.1139)};
\addplot[color={rgb,1:red,0.700;green,0.538;blue,0.538}, line width=0.3pt, forget plot] coordinates {(8.600,6.5262) (52.500,11.8867)};
\addplot[color={rgb,1:red,0.284;green,0.284;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.328,2.0974) (57.225,12.6940)};
\addplot[color={rgb,1:red,0.443;green,0.443;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.000,6.3070) (105.900,23.7177)};
\addplot[color={rgb,1:red,0.700;green,0.649;blue,0.649}, line width=0.3pt, forget plot] coordinates {(6.500,4.5213) (65.000,12.5003)};
\addplot[color={rgb,1:red,0.489;green,0.489;blue,0.700}, line width=0.3pt, forget plot] coordinates {(11.888,5.4185) (83.000,17.5165)};
\addplot[color={rgb,1:red,0.700;green,0.655;blue,0.655}, line width=0.3pt, forget plot] coordinates {(6.183,2.7091) (70.675,11.5562)};
\addplot[color={rgb,1:red,0.190;green,0.190;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.714,2.5166) (53.125,12.6167)};
\addplot[color={rgb,1:red,0.401;green,0.401;blue,0.700}, line width=0.3pt, forget plot] coordinates {(10.275,6.9834) (69.675,17.7623)};
\addplot[color={rgb,1:red,0.656;green,0.656;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.100,5.8710) (71.175,15.2421)};
\addplot[color={rgb,1:red,0.700;green,0.658;blue,0.658}, line width=0.3pt, forget plot] coordinates {(7.468,4.9020) (75.000,14.1914)};
\addplot[color={rgb,1:red,0.336;green,0.336;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.055,4.6951) (72.500,17.3072)};
\addplot[color={rgb,1:red,0.700;green,0.586;blue,0.586}, line width=0.3pt, forget plot] coordinates {(5.742,4.0893) (45.437,9.1827)};
\addplot[color={rgb,1:red,0.700;green,0.626;blue,0.626}, line width=0.3pt, forget plot] coordinates {(2.052,1.3190) (17.225,3.3435)};
\addplot[color={rgb,1:red,0.594;green,0.594;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.555,5.1028) (47.000,11.4365)};
\addplot[color={rgb,1:red,0.700;green,0.661;blue,0.661}, line width=0.3pt, forget plot] coordinates {(6.955,5.3625) (64.725,13.3316)};
\addplot[color={rgb,1:red,0.582;green,0.582;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.555,2.7136) (33.450,7.1238)};
\addplot[color={rgb,1:red,0.579;green,0.579;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.678,2.9275) (66.872,12.4738)};
\addplot[color={rgb,1:red,0.487;green,0.487;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.100,4.2374) (52.225,12.0954)};
\addplot[color={rgb,1:red,0.514;green,0.514;blue,0.700}, line width=0.3pt, forget plot] coordinates {(1.928,1.0245) (10.225,2.4094)};
\addplot[color={rgb,1:red,0.338;green,0.338;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.500,2.1358) (32.187,7.5748)};
\addplot[color={rgb,1:red,0.205;green,0.205;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.600,1.9154) (22.112,5.7427)};
\addplot[color={rgb,1:red,0.401;green,0.401;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.600,2.8389) (55.374,11.8732)};
\addplot[color={rgb,1:red,0.508;green,0.508;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.178,3.7705) (72.225,14.6763)};
\addplot[color={rgb,1:red,0.700;green,0.536;blue,0.536}, line width=0.3pt, forget plot] coordinates {(18.000,6.8204) (79.175,14.2740)};
\addplot[color={rgb,1:red,0.133;green,0.133;blue,0.700}, line width=0.3pt, forget plot] coordinates {(12.888,6.5785) (133.900,32.7218)};
\addplot[color={rgb,1:red,0.592;green,0.592;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.388,2.0315) (61.612,11.0105)};
\addplot[color={rgb,1:red,0.109;green,0.109;blue,0.700}, line width=0.3pt, forget plot] coordinates {(21.774,12.9959) (327.250,79.9510)};
\addplot[color={rgb,1:red,0.700;green,0.412;blue,0.412}, line width=0.3pt, forget plot] coordinates {(3.600,2.5550) (34.725,5.8488)};
\addplot[color={rgb,1:red,0.700;green,0.657;blue,0.657}, line width=0.3pt, forget plot] coordinates {(5.296,3.4018) (38.450,7.9581)};
\addplot[color={rgb,1:red,0.700;green,0.496;blue,0.496}, line width=0.3pt, forget plot] coordinates {(1.868,0.8845) (10.000,1.8327)};
\addplot[color={rgb,1:red,0.108;green,0.108;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.655,7.0496) (108.450,28.9343)};
\addplot[color={rgb,1:red,0.658;green,0.658;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.500,2.1518) (22.500,4.9705)};
\addplot[color={rgb,1:red,0.559;green,0.559;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.288,4.2303) (76.500,15.3806)};
\addplot[color={rgb,1:red,0.411;green,0.411;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.655,2.6863) (41.368,9.4813)};
\addplot[color={rgb,1:red,0.313;green,0.313;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.448,3.8194) (70.900,16.2474)};
\addplot[color={rgb,1:red,0.104;green,0.104;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.910,8.3592) (145.600,38.4057)};
\addplot[color={rgb,1:red,0.650;green,0.650;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.628,3.6344) (60.225,11.6399)};
\addplot[color={rgb,1:red,0.700;green,0.478;blue,0.478}, line width=0.3pt, forget plot] coordinates {(4.600,1.9349) (49.400,7.0544)};
\addplot[color={rgb,1:red,0.588;green,0.588;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.478,5.6784) (78.450,16.6869)};
\addplot[color={rgb,1:red,0.700;green,0.692;blue,0.692}, line width=0.3pt, forget plot] coordinates {(8.478,5.4228) (58.225,12.4834)};
\addplot[color={rgb,1:red,0.264;green,0.264;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.255,2.3783) (34.950,8.6895)};
\addplot[color={rgb,1:red,0.548;green,0.548;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.100,3.0217) (41.125,9.0396)};
\addplot[color={rgb,1:red,0.700;green,0.396;blue,0.396}, line width=0.3pt, forget plot] coordinates {(5.500,3.8278) (42.112,7.6270)};
\addplot[color={rgb,1:red,0.697;green,0.697;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.188,1.8008) (18.420,4.1272)};
\addplot[color={rgb,1:red,0.502;green,0.502;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.683,6.4953) (80.225,18.7172)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.900,5.4737) (122.300,33.9528)};
\addplot[color={rgb,1:red,0.700;green,0.598;blue,0.598}, line width=0.3pt, forget plot] coordinates {(6.603,4.1871) (40.614,8.6011)};
\addplot[color={rgb,1:red,0.413;green,0.413;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.742,3.4418) (48.000,11.0468)};
\addplot[color={rgb,1:red,0.168;green,0.168;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.910,5.1866) (116.450,28.5634)};
\addplot[color={rgb,1:red,0.122;green,0.122;blue,0.700}, line width=0.3pt, forget plot] coordinates {(13.001,10.6843) (162.300,43.1561)};
\addplot[color={rgb,1:red,0.618;green,0.618;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.355,2.8138) (43.638,9.0002)};
\addplot[color={rgb,1:red,0.633;green,0.633;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.555,3.1120) (47.950,9.5393)};
\addplot[color={rgb,1:red,0.700;green,0.593;blue,0.593}, line width=0.3pt, forget plot] coordinates {(4.778,2.5774) (39.140,7.0166)};
\addplot[color={rgb,1:red,0.700;green,0.663;blue,0.663}, line width=0.3pt, forget plot] coordinates {(1.925,1.4228) (10.612,2.6227)};
\addplot[color={rgb,1:red,0.630;green,0.630;blue,0.700}, line width=0.3pt, forget plot] coordinates {(1.892,1.0963) (10.000,2.3284)};
\addplot[color={rgb,1:red,0.304;green,0.304;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.210,5.2229) (81.495,19.4372)};
\addplot[color={rgb,1:red,0.539;green,0.539;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.600,1.9978) (29.725,6.2732)};
\addplot[color={rgb,1:red,0.700;green,0.658;blue,0.658}, line width=0.3pt, forget plot] coordinates {(6.986,3.7812) (59.450,10.9976)};
\addplot[color={rgb,1:red,0.502;green,0.502;blue,0.700}, line width=0.3pt, forget plot] coordinates {(18.500,9.0528) (124.450,26.9013)};
\addplot[color={rgb,1:red,0.700;green,0.672;blue,0.672}, line width=0.3pt, forget plot] coordinates {(20.049,9.3834) (108.450,21.7012)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.755,2.9691) (40.112,11.9267)};
\addplot[color={rgb,1:red,0.489;green,0.489;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.600,3.8836) (48.338,11.3251)};
\addplot[color={rgb,1:red,0.311;green,0.311;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.355,7.7007) (112.250,27.7651)};
\addplot[color={rgb,1:red,0.346;green,0.346;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.101,3.5726) (56.400,13.4323)};
\addplot[color={rgb,1:red,0.353;green,0.353;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.100,4.4263) (66.000,15.6681)};
\addplot[color={rgb,1:red,0.634;green,0.634;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.555,3.8589) (60.575,12.1946)};
\addplot[color={rgb,1:red,0.390;green,0.390;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.600,1.9813) (51.350,10.7159)};
\addplot[color={rgb,1:red,0.430;green,0.430;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.000,3.8669) (40.000,10.2677)};
\addplot[color={rgb,1:red,0.423;green,0.423;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.543,3.8020) (38.943,10.1252)};
\addplot[color={rgb,1:red,0.343;green,0.343;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.500,4.4363) (77.175,17.6003)};
\addplot[color={rgb,1:red,0.552;green,0.552;blue,0.700}, line width=0.3pt, forget plot] coordinates {(11.775,7.9826) (212.900,40.5599)};
\addplot[color={rgb,1:red,0.647;green,0.647;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.500,1.7512) (24.000,4.9721)};
\addplot[color={rgb,1:red,0.700;green,0.690;blue,0.690}, line width=0.3pt, forget plot] coordinates {(1.800,0.7575) (10.000,1.9187)};
\addplot[color={rgb,1:red,0.052;green,0.052;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.142,1.9733) (21.112,6.2693)};
\addplot[color={rgb,1:red,0.537;green,0.537;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.500,5.4406) (52.225,12.6103)};
\addplot[color={rgb,1:red,0.635;green,0.635;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.578,1.9183) (34.500,6.5979)};
\addplot[color={rgb,1:red,0.700;green,0.618;blue,0.618}, line width=0.3pt, forget plot] coordinates {(5.783,4.5379) (60.450,11.7730)};
\addplot[color={rgb,1:red,0.700;green,0.476;blue,0.476}, line width=0.3pt, forget plot] coordinates {(3.778,2.9854) (36.250,6.6900)};
\addplot[color={rgb,1:red,0.383;green,0.383;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.142,1.0777) (16.500,3.7176)};
\addplot[color={rgb,1:red,0.547;green,0.547;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.555,4.5065) (58.725,12.9938)};
\addplot[color={rgb,1:red,0.427;green,0.427;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.024,3.1954) (36.000,8.7137)};
\addplot[color={rgb,1:red,0.689;green,0.689;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.555,4.1751) (54.362,11.0750)};
\addplot[color={rgb,1:red,0.700;green,0.627;blue,0.627}, line width=0.3pt, forget plot] coordinates {(3.355,2.4888) (31.450,6.2396)};
\addplot[color={rgb,1:red,0.603;green,0.603;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.255,4.1706) (65.225,13.4933)};
\addplot[color={rgb,1:red,0.700;green,0.478;blue,0.478}, line width=0.3pt, forget plot] coordinates {(4.357,2.5776) (35.502,6.1381)};
\addplot[color={rgb,1:red,0.453;green,0.453;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.300,3.4775) (59.450,12.9411)};
\addplot[color={rgb,1:red,0.527;green,0.527;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.000,1.3441) (17.750,3.7819)};
\addplot[color={rgb,1:red,0.342;green,0.342;blue,0.700}, line width=0.3pt, forget plot] coordinates {(9.178,5.9097) (69.675,17.3484)};
\addplot[color={rgb,1:red,0.694;green,0.694;blue,0.700}, line width=0.3pt, forget plot] coordinates {(11.263,7.8174) (84.225,18.2999)};
\addplot[color={rgb,1:red,0.508;green,0.508;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.478,2.7676) (32.362,7.2755)};
\addplot[color={rgb,1:red,0.558;green,0.558;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.555,3.1615) (72.000,13.8765)};
\addplot[color={rgb,1:red,0.192;green,0.192;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.255,3.7708) (85.000,20.3873)};
\addplot[color={rgb,1:red,0.295;green,0.295;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.800,4.0227) (51.026,12.8470)};
\addplot[color={rgb,1:red,0.622;green,0.622;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.700,2.0678) (25.030,5.3308)};
\addplot[color={rgb,1:red,0.700;green,0.537;blue,0.537}, line width=0.3pt, forget plot] coordinates {(6.655,4.1859) (37.913,7.9991)};
\addplot[color={rgb,1:red,0.700;green,0.546;blue,0.546}, line width=0.3pt, forget plot] coordinates {(7.910,5.5584) (45.000,10.1227)};
\addplot[color={rgb,1:red,0.535;green,0.535;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.000,3.2546) (39.022,8.8437)};
\addplot[color={rgb,1:red,0.672;green,0.672;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.828,2.1361) (29.612,5.9144)};
\addplot[color={rgb,1:red,0.668;green,0.668;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.255,4.6374) (55.400,11.7180)};
\addplot[color={rgb,1:red,0.533;green,0.533;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.378,3.4630) (44.725,9.7689)};
\addplot[color={rgb,1:red,0.700;green,0.664;blue,0.664}, line width=0.3pt, forget plot] coordinates {(7.600,5.3108) (66.950,13.5201)};
\addplot[color={rgb,1:red,0.439;green,0.439;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.310,2.2393) (35.862,7.9881)};
\addplot[color={rgb,1:red,0.508;green,0.508;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.355,3.6259) (49.112,10.9664)};
\addplot[color={rgb,1:red,0.700;green,0.516;blue,0.516}, line width=0.3pt, forget plot] coordinates {(4.300,2.1961) (30.629,5.3352)};
\addplot[color={rgb,1:red,0.586;green,0.586;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.500,2.1332) (24.450,5.4360)};
\addplot[color={rgb,1:red,0.452;green,0.452;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.900,1.3831) (15.500,3.5875)};
\addplot[color={rgb,1:red,0.020;green,0.020;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.700,3.6103) (67.452,18.0775)};
\addplot[color={rgb,1:red,0.686;green,0.686;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.400,1.7059) (22.142,4.4184)};
\addplot[color={rgb,1:red,0.700;green,0.655;blue,0.655}, line width=0.3pt, forget plot] coordinates {(19.861,8.9186) (102.411,20.2369)};
\addplot[color={rgb,1:red,0.111;green,0.111;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.778,2.0569) (33.112,8.4758)};
\addplot[color={rgb,1:red,0.700;green,0.553;blue,0.553}, line width=0.3pt, forget plot] coordinates {(7.600,5.2963) (43.337,9.7283)};
\addplot[color={rgb,1:red,0.700;green,0.368;blue,0.368}, line width=0.3pt, forget plot] coordinates {(7.155,4.7475) (40.090,8.0479)};
\addplot[color={rgb,1:red,0.700;green,0.591;blue,0.591}, line width=0.3pt, forget plot] coordinates {(3.600,2.1339) (25.315,4.9329)};
\addplot[color={rgb,1:red,0.477;green,0.477;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.055,2.1885) (26.112,5.9756)};
\addplot[color={rgb,1:red,0.700;green,0.355;blue,0.355}, line width=0.3pt, forget plot] coordinates {(3.055,1.9299) (20.450,3.6430)};
\addplot[color={rgb,1:red,0.700;green,0.581;blue,0.581}, line width=0.3pt, forget plot] coordinates {(7.955,6.1660) (50.067,11.5396)};
\addplot[color={rgb,1:red,0.442;green,0.442;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.200,1.5337) (30.390,6.3230)};
\addplot[color={rgb,1:red,0.165;green,0.165;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.100,1.5985) (17.862,4.9382)};
\addplot[color={rgb,1:red,0.192;green,0.192;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.900,2.9027) (43.500,11.1583)};
\addplot[color={rgb,1:red,0.678;green,0.678;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.500,2.2074) (22.250,4.9421)};
\addplot[color={rgb,1:red,0.700;green,0.271;blue,0.271}, line width=0.3pt, forget plot] coordinates {(16.960,5.3625) (64.875,9.5618)};
\addplot[color={rgb,1:red,0.632;green,0.632;blue,0.700}, line width=0.3pt, forget plot] coordinates {(11.924,7.0727) (130.160,25.0080)};
\addplot[color={rgb,1:red,0.256;green,0.256;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.201,3.1065) (49.227,11.9195)};
\addplot[color={rgb,1:red,0.422;green,0.422;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.500,1.5822) (20.408,4.6061)};
\addplot[color={rgb,1:red,0.700;green,0.545;blue,0.545}, line width=0.3pt, forget plot] coordinates {(4.620,2.4441) (34.725,6.1455)};
\addplot[color={rgb,1:red,0.323;green,0.323;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.455,3.3838) (38.450,9.7055)};
\addplot[color={rgb,1:red,0.675;green,0.675;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.055,2.5005) (22.725,5.2297)};
\addplot[color={rgb,1:red,0.299;green,0.299;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.878,1.1211) (18.112,4.0854)};
\addplot[color={rgb,1:red,0.700;green,0.674;blue,0.674}, line width=0.3pt, forget plot] coordinates {(22.506,9.5671) (130.900,24.7025)};
\addplot[color={rgb,1:red,0.380;green,0.380;blue,0.700}, line width=0.3pt, forget plot] coordinates {(2.600,1.2954) (33.658,7.0167)};
\addplot[color={rgb,1:red,0.700;green,0.320;blue,0.320}, line width=0.3pt, forget plot] coordinates {(4.041,3.0538) (32.000,5.6822)};
\addplot[color={rgb,1:red,0.700;green,0.694;blue,0.694}, line width=0.3pt, forget plot] coordinates {(6.478,5.8499) (87.950,17.4357)};
\addplot[color={rgb,1:red,0.542;green,0.542;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.986,4.5780) (43.225,10.4988)};
\addplot[color={rgb,1:red,0.700;green,0.497;blue,0.497}, line width=0.3pt, forget plot] coordinates {(9.900,6.2848) (133.790,20.7466)};
\addplot[color={rgb,1:red,0.300;green,0.300;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.100,6.2819) (104.000,25.1257)};
\addplot[color={rgb,1:red,0.637;green,0.637;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.955,4.4975) (54.400,11.8167)};
\addplot[color={rgb,1:red,0.700;green,0.510;blue,0.510}, line width=0.3pt, forget plot] coordinates {(5.000,3.3733) (46.725,8.3186)};
\addplot[color={rgb,1:red,0.584;green,0.584;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.700,2.5085) (35.726,7.5653)};
\addplot[color={rgb,1:red,0.479;green,0.479;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.278,1.7132) (32.950,6.7999)};
\addplot[color={rgb,1:red,0.700;green,0.577;blue,0.577}, line width=0.3pt, forget plot] coordinates {(4.078,2.7444) (32.946,6.4153)};
\addplot[color={rgb,1:red,0.467;green,0.467;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.600,4.4057) (59.175,13.6764)};
\addplot[color={rgb,1:red,0.700;green,0.620;blue,0.620}, line width=0.3pt, forget plot] coordinates {(3.500,1.7385) (26.725,4.8181)};
\addplot[color={rgb,1:red,0.700;green,0.568;blue,0.568}, line width=0.3pt, forget plot] coordinates {(5.500,3.9555) (42.362,8.5978)};
\addplot[color={rgb,1:red,0.626;green,0.626;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.600,4.1674) (43.175,9.8961)};
\addplot[color={rgb,1:red,0.568;green,0.568;blue,0.700}, line width=0.3pt, forget plot] coordinates {(20.833,9.5043) (126.000,26.3238)};
\addplot[color={rgb,1:red,0.613;green,0.613;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.100,2.4896) (49.762,9.5283)};
\addplot[color={rgb,1:red,0.577;green,0.577;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.628,2.8742) (43.189,8.9968)};
\addplot[color={rgb,1:red,0.700;green,0.683;blue,0.683}, line width=0.3pt, forget plot] coordinates {(3.500,1.7606) (31.460,5.6959)};
\addplot[color={rgb,1:red,0.700;green,0.543;blue,0.543}, line width=0.3pt, forget plot] coordinates {(3.555,2.0214) (22.311,4.3236)};
\addplot[color={rgb,1:red,0.700;green,0.542;blue,0.542}, line width=0.3pt, forget plot] coordinates {(5.055,3.6692) (42.862,8.3054)};
\addplot[color={rgb,1:red,0.700;green,0.560;blue,0.560}, line width=0.3pt, forget plot] coordinates {(7.410,5.6459) (53.232,11.3688)};
\addplot[color={rgb,1:red,0.700;green,0.634;blue,0.634}, line width=0.3pt, forget plot] coordinates {(4.778,3.2843) (47.500,9.0287)};
\addplot[color={rgb,1:red,0.700;green,0.456;blue,0.456}, line width=0.3pt, forget plot] coordinates {(8.101,7.9128) (66.225,14.3925)};
\addplot[color={rgb,1:red,0.700;green,0.419;blue,0.419}, line width=0.3pt, forget plot] coordinates {(6.100,4.4904) (78.350,12.2022)};
\addplot[color={rgb,1:red,0.566;green,0.566;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.600,4.2984) (43.000,10.2927)};
\addplot[color={rgb,1:red,0.700;green,0.397;blue,0.397}, line width=0.3pt, forget plot] coordinates {(4.678,3.4104) (38.000,6.8726)};
\addplot[color={rgb,1:red,0.700;green,0.450;blue,0.450}, line width=0.3pt, forget plot] coordinates {(23.750,10.8374) (132.728,22.9012)};
\addplot[color={rgb,1:red,0.700;green,0.684;blue,0.684}, line width=0.3pt, forget plot] coordinates {(3.800,2.5114) (25.250,5.5346)};
\addplot[color={rgb,1:red,0.589;green,0.589;blue,0.700}, line width=0.3pt, forget plot] coordinates {(12.950,7.9469) (287.800,51.1592)};
\addplot[color={rgb,1:red,0.410;green,0.410;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.800,3.9346) (56.960,13.1608)};
\addplot[color={rgb,1:red,0.485;green,0.485;blue,0.700}, line width=0.3pt, forget plot] coordinates {(8.055,6.6067) (107.900,23.6508)};
\addplot[color={rgb,1:red,0.419;green,0.419;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.200,5.9089) (76.225,18.4580)};
\addplot[color={rgb,1:red,0.452;green,0.452;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.500,3.3403) (39.862,9.3521)};
\addplot[color={rgb,1:red,0.681;green,0.681;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.069,2.7404) (25.755,5.8944)};
\addplot[color={rgb,1:red,0.700;green,0.342;blue,0.342}, line width=0.3pt, forget plot] coordinates {(5.455,3.0703) (32.612,5.6978)};
\addplot[color={rgb,1:red,0.395;green,0.395;blue,0.700}, line width=0.3pt, forget plot] coordinates {(15.888,9.3531) (177.316,38.7759)};
\addplot[color={rgb,1:red,0.700;green,0.536;blue,0.536}, line width=0.3pt, forget plot] coordinates {(5.355,3.1151) (42.250,7.6107)};
\addplot[color={rgb,1:red,0.636;green,0.636;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.600,2.0834) (32.112,6.3937)};
\addplot[color={rgb,1:red,0.499;green,0.499;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.990,4.4460) (76.626,16.3772)};
\addplot[color={rgb,1:red,0.700;green,0.543;blue,0.543}, line width=0.3pt, forget plot] coordinates {(20.089,8.9642) (119.350,21.1421)};
\addplot[color={rgb,1:red,0.700;green,0.679;blue,0.679}, line width=0.3pt, forget plot] coordinates {(3.460,1.2588) (16.112,3.0339)};
\addplot[color={rgb,1:red,0.700;green,0.571;blue,0.571}, line width=0.3pt, forget plot] coordinates {(4.726,2.9959) (40.755,7.5475)};
\addplot[color={rgb,1:red,0.700;green,0.556;blue,0.556}, line width=0.3pt, forget plot] coordinates {(4.370,2.0761) (23.362,4.4385)};
\addplot[color={rgb,1:red,0.700;green,0.557;blue,0.557}, line width=0.3pt, forget plot] coordinates {(6.500,5.2822) (93.575,16.1243)};
\addplot[color={rgb,1:red,0.700;green,0.491;blue,0.491}, line width=0.3pt, forget plot] coordinates {(4.055,1.5651) (16.750,3.0371)};
\addplot[color={rgb,1:red,0.450;green,0.450;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.897,2.5613) (36.704,8.1325)};
\addplot[color={rgb,1:red,0.687;green,0.687;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.055,5.2870) (80.725,15.9441)};
\addplot[color={rgb,1:red,0.295;green,0.295;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.000,5.3178) (86.400,20.8173)};
\addplot[color={rgb,1:red,0.697;green,0.697;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.355,2.7747) (40.362,7.9337)};
\addplot[color={rgb,1:red,0.700;green,0.449;blue,0.449}, line width=0.3pt, forget plot] coordinates {(3.250,1.5814) (15.612,2.9487)};
\addplot[color={rgb,1:red,0.700;green,0.561;blue,0.561}, line width=0.3pt, forget plot] coordinates {(5.176,3.3993) (70.225,11.5306)};
\addplot[color={rgb,1:red,0.700;green,0.652;blue,0.652}, line width=0.3pt, forget plot] coordinates {(5.083,3.5079) (56.362,10.5191)};
\addplot[color={rgb,1:red,0.270;green,0.270;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.937,5.2386) (93.400,22.3865)};
\addplot[color={rgb,1:red,0.683;green,0.683;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.614,5.2328) (48.037,11.1018)};
\addplot[color={rgb,1:red,0.527;green,0.527;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.327,3.0650) (57.355,11.6649)};
\addplot[color={rgb,1:red,0.267;green,0.267;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.100,5.0948) (79.900,19.5670)};
\addplot[color={rgb,1:red,0.700;green,0.392;blue,0.392}, line width=0.3pt, forget plot] coordinates {(6.850,6.1982) (129.388,18.8456)};
\addplot[color={rgb,1:red,0.700;green,0.523;blue,0.523}, line width=0.3pt, forget plot] coordinates {(5.176,3.3938) (39.950,7.5723)};
\addplot[color={rgb,1:red,0.583;green,0.583;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.310,3.4903) (68.000,13.4008)};
\addplot[color={rgb,1:red,0.700;green,0.397;blue,0.397}, line width=0.3pt, forget plot] coordinates {(5.700,4.0849) (34.725,7.1018)};
\addplot[color={rgb,1:red,0.668;green,0.668;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.455,3.2807) (40.250,8.5464)};
\addplot[color={rgb,1:red,0.584;green,0.584;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.933,3.9028) (49.950,11.0129)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.110,5.0490) (82.225,24.9106)};
\addplot[color={rgb,1:red,0.492;green,0.492;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.255,2.1611) (47.840,9.5608)};
\addplot[color={rgb,1:red,0.432;green,0.432;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.828,2.9109) (37.950,8.7886)};
\addplot[color={rgb,1:red,0.465;green,0.465;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.166,3.2901) (58.450,12.5208)};
\addplot[color={rgb,1:red,0.700;green,0.661;blue,0.661}, line width=0.3pt, forget plot] coordinates {(5.600,4.0655) (56.225,11.0451)};
\addplot[color={rgb,1:red,0.688;green,0.688;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.683,3.0441) (25.000,5.9786)};
\addplot[color={rgb,1:red,0.700;green,0.542;blue,0.542}, line width=0.3pt, forget plot] coordinates {(5.210,3.9638) (67.725,11.6313)};
\addplot[color={rgb,1:red,0.344;green,0.344;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.600,2.3167) (42.225,9.4221)};
\addplot[color={rgb,1:red,0.700;green,0.620;blue,0.620}, line width=0.3pt, forget plot] coordinates {(4.155,2.8088) (32.956,6.6299)};
\addplot[color={rgb,1:red,0.665;green,0.665;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.600,3.5732) (55.000,10.8576)};
\addplot[color={rgb,1:red,0.401;green,0.401;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.600,2.8308) (36.785,8.6726)};
\addplot[color={rgb,1:red,0.700;green,0.116;blue,0.116}, line width=0.3pt, forget plot] coordinates {(5.105,3.2535) (23.112,4.4725)};
\addplot[color={rgb,1:red,0.700;green,0.654;blue,0.654}, line width=0.3pt, forget plot] coordinates {(5.100,3.4738) (44.725,8.9009)};
\addplot[color={rgb,1:red,0.458;green,0.458;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.978,4.5346) (66.175,15.0208)};
\addplot[color={rgb,1:red,0.700;green,0.674;blue,0.674}, line width=0.3pt, forget plot] coordinates {(4.600,2.5822) (45.112,8.2402)};
\addplot[color={rgb,1:red,0.482;green,0.482;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.300,2.3462) (40.500,8.5388)};
\addplot[color={rgb,1:red,0.621;green,0.621;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.328,5.1294) (76.176,15.6712)};
\addplot[color={rgb,1:red,0.700;green,0.599;blue,0.599}, line width=0.3pt, forget plot] coordinates {(4.300,2.5979) (63.000,10.2282)};
\addplot[color={rgb,1:red,0.526;green,0.526;blue,0.700}, line width=0.3pt, forget plot] coordinates {(6.800,4.7545) (88.900,18.3335)};
\addplot[color={rgb,1:red,0.700;green,0.180;blue,0.180}, line width=0.3pt, forget plot] coordinates {(8.100,4.6115) (80.225,10.0867)};
\addplot[color={rgb,1:red,0.034;green,0.034;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.800,4.9137) (104.900,28.0459)};
\addplot[color={rgb,1:red,0.700;green,0.395;blue,0.395}, line width=0.3pt, forget plot] coordinates {(7.100,4.6921) (54.995,9.6577)};
\addplot[color={rgb,1:red,0.700;green,0.363;blue,0.363}, line width=0.3pt, forget plot] coordinates {(6.100,5.0313) (41.112,8.5151)};
\addplot[color={rgb,1:red,0.700;green,0.626;blue,0.626}, line width=0.3pt, forget plot] coordinates {(6.455,5.2176) (81.280,15.1997)};
\addplot[color={rgb,1:red,0.700;green,0.418;blue,0.418}, line width=0.3pt, forget plot] coordinates {(4.128,2.0561) (22.612,4.0274)};
\addplot[color={rgb,1:red,0.700;green,0.674;blue,0.674}, line width=0.3pt, forget plot] coordinates {(4.100,1.6640) (20.000,3.8840)};
\addplot[color={rgb,1:red,0.700;green,0.560;blue,0.560}, line width=0.3pt, forget plot] coordinates {(4.700,2.9514) (34.725,6.6999)};
\addplot[color={rgb,1:red,0.700;green,0.663;blue,0.663}, line width=0.3pt, forget plot] coordinates {(7.155,5.3454) (80.225,15.4408)};
\addplot[color={rgb,1:red,0.700;green,0.596;blue,0.596}, line width=0.3pt, forget plot] coordinates {(6.055,3.6084) (81.950,13.4450)};
\addplot[color={rgb,1:red,0.700;green,0.620;blue,0.620}, line width=0.3pt, forget plot] coordinates {(6.600,3.8628) (76.176,13.0903)};
\addplot[color={rgb,1:red,0.700;green,0.450;blue,0.450}, line width=0.3pt, forget plot] coordinates {(5.259,2.9750) (26.000,5.2725)};
\addplot[color={rgb,1:red,0.700;green,0.117;blue,0.117}, line width=0.3pt, forget plot] coordinates {(16.960,5.8277) (82.225,10.2563)};
\addplot[color={rgb,1:red,0.700;green,0.685;blue,0.685}, line width=0.3pt, forget plot] coordinates {(4.370,2.8470) (26.500,5.9670)};
\addplot[color={rgb,1:red,0.661;green,0.661;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.100,2.0084) (34.175,6.4604)};
\addplot[color={rgb,1:red,0.700;green,0.274;blue,0.274}, line width=0.3pt, forget plot] coordinates {(7.478,4.5135) (52.057,8.4371)};
\addplot[color={rgb,1:red,0.700;green,0.353;blue,0.353}, line width=0.3pt, forget plot] coordinates {(5.600,3.0202) (30.725,5.4879)};
\addplot[color={rgb,1:red,0.700;green,0.444;blue,0.444}, line width=0.3pt, forget plot] coordinates {(4.000,2.1127) (24.500,4.3673)};
\addplot[color={rgb,1:red,0.700;green,0.331;blue,0.331}, line width=0.3pt, forget plot] coordinates {(5.178,3.6554) (28.725,5.9012)};
\addplot[color={rgb,1:red,0.700;green,0.490;blue,0.490}, line width=0.3pt, forget plot] coordinates {(5.200,3.9218) (31.587,6.9789)};
\addplot[color={rgb,1:red,0.700;green,0.467;blue,0.467}, line width=0.3pt, forget plot] coordinates {(4.378,2.1664) (36.950,5.8462)};
\addplot[color={rgb,1:red,0.700;green,0.643;blue,0.643}, line width=0.3pt, forget plot] coordinates {(4.996,2.8341) (29.452,6.1502)};
\addplot[color={rgb,1:red,0.700;green,0.122;blue,0.122}, line width=0.3pt, forget plot] coordinates {(11.000,5.8464) (88.725,11.1669)};
\addplot[color={rgb,1:red,0.700;green,0.219;blue,0.219}, line width=0.3pt, forget plot] coordinates {(5.100,2.9599) (43.430,6.0645)};
\addplot[color={rgb,1:red,0.570;green,0.570;blue,0.700}, line width=0.3pt, forget plot] coordinates {(5.749,2.7707) (75.225,13.8666)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(15.525,4.8984) (78.710,8.1619)};
\addplot[color={rgb,1:red,0.700;green,0.170;blue,0.170}, line width=0.3pt, forget plot] coordinates {(8.055,4.9341) (58.287,8.6809)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(6.600,4.1575) (45.560,5.1802)};
\addplot[color={rgb,1:red,0.700;green,0.109;blue,0.109}, line width=0.3pt, forget plot] coordinates {(4.773,2.2260) (23.725,3.4926)};
\addplot[color={rgb,1:red,0.700;green,0.055;blue,0.055}, line width=0.3pt, forget plot] coordinates {(5.817,3.5326) (42.500,5.7269)};
\addplot[color={rgb,1:red,0.700;green,0.044;blue,0.044}, line width=0.3pt, forget plot] coordinates {(6.655,3.5900) (36.293,5.3216)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(4.908,2.4280) (22.225,3.0520)};
\addplot[color={rgb,1:red,0.700;green,0.064;blue,0.064}, line width=0.3pt, forget plot] coordinates {(5.100,2.4815) (31.612,4.0974)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(13.000,6.4075) (72.000,8.0500)};
\addplot[color={rgb,1:red,0.700;green,0.124;blue,0.124}, line width=0.3pt, forget plot] coordinates {(5.871,2.8893) (33.837,4.8123)};
\addplot[color={rgb,1:red,0.700;green,0.020;blue,0.020}, line width=0.3pt, forget plot] coordinates {(7.000,3.5644) (35.747,5.1556)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(9.510,5.3066) (126.900,11.2225)};
\addplot[color={rgb,1:red,0.700;green,0.303;blue,0.303}, line width=0.3pt, forget plot] coordinates {(17.888,10.2012) (281.800,34.4234)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(5.278,3.2591) (24.114,4.1014)};
\addplot[color={rgb,1:red,0.700;green,0.234;blue,0.234}, line width=0.3pt, forget plot] coordinates {(5.600,2.9309) (45.000,6.1946)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(9.855,5.4340) (61.998,5.7210)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(14.885,5.5171) (76.225,6.8641)};
\addplot[color={rgb,1:red,0.700;green,0.538;blue,0.538}, line width=0.3pt, forget plot] coordinates {(6.600,3.0281) (46.000,7.8366)};
\addplot[color={rgb,1:red,0.700;green,0.202;blue,0.202}, line width=0.3pt, forget plot] coordinates {(6.941,3.5027) (40.900,6.1762)};
\addplot[color={rgb,1:red,0.700;green,0.675;blue,0.675}, line width=0.3pt, forget plot] coordinates {(6.333,3.3526) (70.900,12.3712)};
\addplot[color={rgb,1:red,0.700;green,0.204;blue,0.204}, line width=0.3pt, forget plot] coordinates {(6.555,2.8423) (36.022,5.1720)};
\addplot[color={rgb,1:red,0.700;green,0.055;blue,0.055}, line width=0.3pt, forget plot] coordinates {(14.877,8.7056) (90.792,13.2476)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(12.530,6.8021) (76.225,6.7801)};
\addplot[color={rgb,1:red,0.700;green,0.017;blue,0.017}, line width=0.3pt, forget plot] coordinates {(16.750,8.5246) (134.747,14.9998)};
\addplot[color={rgb,1:red,0.700;green,0.104;blue,0.104}, line width=0.3pt, forget plot] coordinates {(6.000,3.4666) (25.252,4.7400)};
\addplot[color={rgb,1:red,0.700;green,0.027;blue,0.027}, line width=0.3pt, forget plot] coordinates {(11.960,5.9825) (71.225,9.3150)};
\addplot[color={rgb,1:red,0.700;green,0.109;blue,0.109}, line width=0.3pt, forget plot] coordinates {(6.155,3.5866) (42.925,6.0401)};
\addplot[color={rgb,1:red,0.700;green,0.048;blue,0.048}, line width=0.3pt, forget plot] coordinates {(5.100,2.2357) (27.000,3.5262)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(6.989,4.1042) (41.725,5.8684)};
\addplot[color={rgb,1:red,0.700;green,0.081;blue,0.081}, line width=0.3pt, forget plot] coordinates {(8.628,4.7037) (75.025,8.8940)};
\addplot[color={rgb,1:red,0.700;green,0.178;blue,0.178}, line width=0.3pt, forget plot] coordinates {(6.228,2.8141) (30.752,4.6692)};
\addplot[color={rgb,1:red,0.700;green,0.069;blue,0.069}, line width=0.3pt, forget plot] coordinates {(7.155,5.1316) (62.225,8.5234)};
\addplot[color={rgb,1:red,0.700;green,0.071;blue,0.071}, line width=0.3pt, forget plot] coordinates {(6.155,3.5417) (53.075,6.4427)};
\addplot[color={rgb,1:red,0.700;green,0.243;blue,0.243}, line width=0.3pt, forget plot] coordinates {(15.996,8.3017) (111.446,16.3283)};
\addplot[color={rgb,1:red,0.700;green,0.351;blue,0.351}, line width=0.3pt, forget plot] coordinates {(11.000,6.8154) (109.450,16.4572)};
\addplot[color={rgb,1:red,0.700;green,0.039;blue,0.039}, line width=0.3pt, forget plot] coordinates {(9.101,4.7338) (70.450,8.2791)};
\addplot[color={rgb,1:red,0.700;green,0.443;blue,0.443}, line width=0.3pt, forget plot] coordinates {(7.500,4.4783) (70.225,11.3685)};
\addplot[color={rgb,1:red,0.700;green,0.487;blue,0.487}, line width=0.3pt, forget plot] coordinates {(12.388,6.1562) (143.625,21.3080)};
\addplot[color={rgb,1:red,0.700;green,0.302;blue,0.302}, line width=0.3pt, forget plot] coordinates {(23.888,7.5745) (160.000,20.0442)};
\addplot[color={rgb,1:red,0.700;green,0.458;blue,0.458}, line width=0.3pt, forget plot] coordinates {(9.500,4.9190) (159.350,21.6651)};
\addplot[color={rgb,1:red,0.700;green,0.438;blue,0.438}, line width=0.3pt, forget plot] coordinates {(11.888,5.8573) (128.450,18.5824)};
\addplot[color={rgb,1:red,0.265;green,0.265;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.138,3.5387) (57.725,14.4026)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(10.404,4.2599) (80.500,7.7577)};
\addplot[color={rgb,1:red,0.700;green,0.317;blue,0.317}, line width=0.3pt, forget plot] coordinates {(12.800,7.5714) (174.350,22.7001)};
\addplot[color={rgb,1:red,0.700;green,0.099;blue,0.099}, line width=0.3pt, forget plot] coordinates {(27.638,9.1363) (251.000,23.7722)};
\addplot[color={rgb,1:red,0.700;green,0.577;blue,0.577}, line width=0.3pt, forget plot] coordinates {(21.388,9.0820) (189.900,30.5096)};
\addplot[color={rgb,1:red,0.700;green,0.350;blue,0.350}, line width=0.3pt, forget plot] coordinates {(16.528,5.7454) (95.000,13.4215)};
\addplot[color={rgb,1:red,0.700;green,0.103;blue,0.103}, line width=0.3pt, forget plot] coordinates {(8.448,5.9056) (133.900,14.1848)};
\addplot[color={rgb,1:red,0.700;green,0.068;blue,0.068}, line width=0.3pt, forget plot] coordinates {(26.075,10.1650) (255.900,24.3075)};
\addplot[color={rgb,1:red,0.700;green,0.123;blue,0.123}, line width=0.3pt, forget plot] coordinates {(5.860,2.9749) (59.000,6.6209)};
\addplot[color={rgb,1:red,0.700;green,0.301;blue,0.301}, line width=0.3pt, forget plot] coordinates {(21.219,7.1140) (130.000,17.0663)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(6.555,3.5397) (59.725,5.5824)};
\addplot[color={rgb,1:red,0.700;green,0.152;blue,0.152}, line width=0.3pt, forget plot] coordinates {(13.000,6.4778) (91.950,12.1876)};
\addplot[color={rgb,1:red,0.652;green,0.652;blue,0.700}, line width=0.3pt, forget plot] coordinates {(4.017,2.3509) (36.500,7.1955)};
\addplot[color={rgb,1:red,0.700;green,0.001;blue,0.001}, line width=0.3pt, forget plot] coordinates {(7.455,4.1832) (81.816,8.1172)};
\addplot[color={rgb,1:red,0.700;green,0.292;blue,0.292}, line width=0.3pt, forget plot] coordinates {(20.913,6.4062) (161.000,19.0567)};
\addplot[color={rgb,1:red,0.700;green,0.034;blue,0.034}, line width=0.3pt, forget plot] coordinates {(17.528,6.4087) (156.800,14.3546)};
\addplot[color={rgb,1:red,0.700;green,0.064;blue,0.064}, line width=0.3pt, forget plot] coordinates {(25.250,8.3007) (228.625,20.7105)};
\addplot[color={rgb,1:red,0.700;green,0.454;blue,0.454}, line width=0.3pt, forget plot] coordinates {(17.900,8.5097) (191.995,27.8743)};
\addplot[color={rgb,1:red,0.700;green,0.088;blue,0.088}, line width=0.3pt, forget plot] coordinates {(13.000,5.4060) (122.125,12.4007)};
\addplot[color={rgb,1:red,0.700;green,0.069;blue,0.069}, line width=0.3pt, forget plot] coordinates {(10.182,4.7529) (95.612,10.0222)};
\addplot[color={rgb,1:red,0.700;green,0.062;blue,0.062}, line width=0.3pt, forget plot] coordinates {(12.250,6.1348) (133.585,13.5082)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(35.110,9.6744) (265.000,19.4079)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(7.100,3.5527) (68.500,6.7826)};
\addplot[color={rgb,1:red,0.700;green,0.261;blue,0.261}, line width=0.3pt, forget plot] coordinates {(19.388,7.0686) (170.000,20.0761)};
\addplot[color={rgb,1:red,0.641;green,0.641;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.100,2.2962) (34.450,7.0167)};
\addplot[color={rgb,1:red,0.700;green,0.239;blue,0.239}, line width=0.3pt, forget plot] coordinates {(31.275,10.8194) (403.625,41.9244)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(13.000,5.5579) (98.950,8.7050)};
\addplot[color={rgb,1:red,0.700;green,0.226;blue,0.226}, line width=0.3pt, forget plot] coordinates {(13.500,5.1570) (129.800,14.6818)};
\addplot[color={rgb,1:red,0.700;green,0.608;blue,0.608}, line width=0.3pt, forget plot] coordinates {(28.583,10.8245) (278.900,43.6277)};
\addplot[color={rgb,1:red,0.700;green,0.384;blue,0.384}, line width=0.3pt, forget plot] coordinates {(31.388,10.9048) (300.450,38.4029)};
\addplot[color={rgb,1:red,0.700;green,0.096;blue,0.096}, line width=0.3pt, forget plot] coordinates {(35.503,11.6726) (277.700,27.4283)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(45.275,12.5853) (287.600,22.9148)};
\addplot[color={rgb,1:red,0.700;green,0.235;blue,0.235}, line width=0.3pt, forget plot] coordinates {(27.163,8.2118) (150.450,18.4534)};
\addplot[color={rgb,1:red,0.700;green,0.197;blue,0.197}, line width=0.3pt, forget plot] coordinates {(28.410,9.5232) (216.350,24.2064)};
\addplot[color={rgb,1:red,0.595;green,0.595;blue,0.700}, line width=0.3pt, forget plot] coordinates {(39.555,15.3952) (510.450,89.0927)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(32.828,11.5945) (281.900,23.6897)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(44.525,11.4952) (340.833,26.4245)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(18.000,7.1448) (140.900,13.4531)};
\addplot[color={rgb,1:red,0.697;green,0.697;blue,0.700}, line width=0.3pt, forget plot] coordinates {(7.055,5.0324) (83.890,16.0500)};
\addplot[color={rgb,1:red,0.700;green,0.197;blue,0.197}, line width=0.3pt, forget plot] coordinates {(50.500,13.6550) (573.950,54.5126)};
\addplot[color={rgb,1:red,0.700;green,0.000;blue,0.000}, line width=0.3pt, forget plot] coordinates {(29.500,8.2243) (251.562,18.0714)};
\addplot[color={rgb,1:red,0.700;green,0.261;blue,0.261}, line width=0.3pt, forget plot] coordinates {(14.525,7.3800) (127.700,17.1486)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.418,3.2525) (40.000,12.0035)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(1.378,2.6309) (35.250,11.8820)};
\addplot[color={rgb,1:red,0.700;green,0.526;blue,0.526}, line width=0.3pt, forget plot] coordinates {(13.915,6.5019) (96.987,16.5160)};
\addplot[color={rgb,1:red,0.000;green,0.000;blue,0.700}, line width=0.3pt, forget plot] coordinates {(3.155,2.4137) (63.000,16.7432)};
\addplot[color={rgb,1:red,0.503;green,0.503;blue,0.700}, line width=0.3pt, forget plot] coordinates {(12.025,5.7260) (84.725,17.9601)};
\addplot[color={rgb,1:red,0.008;green,0.008;blue,0.700}, line width=0.3pt, forget plot] coordinates {(1.700,1.9588) (48.005,12.7072)};


==> figures/data/tails_panel_b_boxes.tex <==
% Generated by results_exhibits.py -- do not edit by hand.
% Whiskers at the 5th and 95th percentiles; markup 1/(1 - median xi) printed at right.
\addplot[boxplot prepared={lower whisker=0.0300, lower quartile=0.0714, median=0.1157, upper quartile=0.1641, upper whisker=0.2170, draw position=1}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,1) {1.131};
\addplot[boxplot prepared={lower whisker=0.0626, lower quartile=0.0955, median=0.1181, upper quartile=0.1421, upper whisker=0.1765, draw position=2}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,2) {1.134};
\addplot[boxplot prepared={lower whisker=0.0387, lower quartile=0.0806, median=0.1206, upper quartile=0.1564, upper whisker=0.2025, draw position=3}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,3) {1.137};
\addplot[boxplot prepared={lower whisker=0.0677, lower quartile=0.1069, median=0.1317, upper quartile=0.1522, upper whisker=0.1852, draw position=4}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,4) {1.152};
\addplot[boxplot prepared={lower whisker=0.0631, lower quartile=0.1066, median=0.1349, upper quartile=0.1610, upper whisker=0.2022, draw position=5}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,5) {1.156};
\addplot[boxplot prepared={lower whisker=0.0584, lower quartile=0.1038, median=0.1357, upper quartile=0.1671, upper whisker=0.2089, draw position=6}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,6) {1.157};
\addplot[boxplot prepared={lower whisker=0.0704, lower quartile=0.1035, median=0.1389, upper quartile=0.1797, upper whisker=0.2309, draw position=7}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,7) {1.161};
\addplot[boxplot prepared={lower whisker=0.0588, lower quartile=0.1174, median=0.1466, upper quartile=0.1722, upper whisker=0.2058, draw position=8}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,8) {1.172};
\addplot[boxplot prepared={lower whisker=0.0671, lower quartile=0.1197, median=0.1498, upper quartile=0.1723, upper whisker=0.2002, draw position=9}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,9) {1.176};
\addplot[boxplot prepared={lower whisker=0.1009, lower quartile=0.1334, median=0.1553, upper quartile=0.1827, upper whisker=0.2335, draw position=10}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,10) {1.184};
\addplot[boxplot prepared={lower whisker=0.0589, lower quartile=0.1103, median=0.1582, upper quartile=0.1900, upper whisker=0.2311, draw position=11}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,11) {1.188};
\addplot[boxplot prepared={lower whisker=0.0692, lower quartile=0.1218, median=0.1802, upper quartile=0.2172, upper whisker=0.2530, draw position=12}, fill=white, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,12) {1.220};
\addplot[boxplot prepared={lower whisker=0.0527, lower quartile=0.1050, median=0.1430, upper quartile=0.1759, upper whisker=0.2225, draw position=13}, fill=gray!25, draw=blue!60!black, line width=0.5pt, forget plot] coordinates {};
\node[anchor=west, font=\scriptsize] at (axis cs:0.30,13) {1.167};


==> figures/data/tails_panel_b_labels.tex <==
% Generated by results_exhibits.py -- do not edit by hand.
\pgfplotsset{tails panel b ticks/.style={ytick={1,2,3,4,5,6,7,8,9,10,11,12,13}, yticklabels={Porsche,Toyota,BMW,Jeep,Honda,Ford,Ferrari,Chevrolet,Land Rover,Volkswagen,Mercedes-Benz,Jaguar,All listings}}}


==> figures/data/tails_styles.tex <==
% Generated by results_exhibits.py -- do not edit by hand.
\pgfplotsset{tails panel a meta/.style={point meta min=0.0527, point meta max=0.2332}}

